Generative Modeling of Residuals for Real-Time Risk-Sensitive Safety with Discrete-Time Control Barrier Functions

A key source of brittleness for robotic systems is the presence of model uncertainty and external disturbances. Most existing approaches to robust control either seek to bound the worst-case disturbance (which results in conservative behavior), or to learn a deterministic dynamics model (which is unable to capture uncertain dynamics or disturbances). This work proposes a different approach: training a state-conditioned generative model to represent the distribution of error residuals between the nominal dynamics and the actual system. In particular we introduce the Online Risk-Informed Optimization controller (ORIO), which uses Discrete-Time Control Barrier Functions, combined with a learned, generative disturbance model, to ensure the safety of the system up to some level of risk. We demonstrate our approach in both simulations and hardware, and show our method can learn a disturbance model that is accurate enough to enable risk-sensitive control of a quadrotor flying aggressively with an unmodelled slung load. We use a conditional variational autoencoder (CVAE) to learn a state-conditioned dynamics residual distribution, and find that the resulting probabilistic safety controller, which can be run at 100Hz on an embedded computer, exhibits less conservative behavior while retaining theoretical safety properties.

==> Old/other.tex <==
\begin{align}
    \begin{bmatrix}
        \dot{x} \\
        \dot{q} \\
        \ddot{x}
    \end{bmatrix}   = &  
    \begin{bmatrix}
        \mathbf{0}_{3\times 3} & \mathbf{0}_{3\times 4} & I_3 \\
        & \mathbf{0}_{4 \times 10}\\
        & \mathbf{0}_{3 \times 10} 
    \end{bmatrix}
    \begin{bmatrix}
        x \\ q \\ \dot{x}
    \end{bmatrix} 
    + \begin{bmatrix}
        \mb{0}_{9\times 1}\\
        -g 
    \end{bmatrix}
    + \begin{bmatrix}
        \mathbf{0}_{3\times 4 }\\
        \mathbf{0}_{4 \times 1} &  Q_{4 \times 3 }(q) \\ 
        \frac{1}{m} R(q) \hat{\mathbf{e}}_z & \mathbf{0}_{3 \times 3}
    \end{bmatrix}
    \begin{bmatrix}
        T \\ \Vec{\omega}
    \end{bmatrix}\\
    Q_{4 \times 3}(q)  & \begin{bmatrix}
        q_x & q_y& q_z \\
        q_w & -q_z & q_y \\
        q_z & q_w & - q_x \\
        q_y & q_x & q_w
    \end{bmatrix} , q \in SO(3)
\end{align}

The matrix multiplication $Q(q)\vec{\omega}$ can be equivalently written as the quaternion multiplication $q_\omega \times q $, where $q_\omega = 0 + \omega_x i + \omega_y j + \omega_z k $. 


\subsection{Hardware}




\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
         \hline $\alpha$ & $\P_\textrm{bound}$ & Certainty Equivalent & RSS & True Distribution \\
         \hline 0.9975 & 0.574 & 0.260 & 0.000 &  0.200 \\ 
         \hline 0.9925 & 0.920 & 0.780 & 0.315 & 0.705  \\
         \hline 
    \end{tabular}
    \caption{Sim trials of drone with different $\alpha$ we successfully get closer to the guaranteed bound (reducing conservatism) while retaining the guarantees that are not present in the standard CBF method.}
    \label{tab:my_label}
\end{table}


\subsection{Simulations}

Learn a nonlinear heteroschedastic distribution from trajectory data. 

Learn a nonlinear multimodel distribution from trajectory data. 



Demonstrate that the method can learn the ground truth distributions and use them to keep the system safe (show statistical safety results with Monte Carlo). 

\begin{itemize}
    \item drone dynamics
    \item trajectory (dagger?) sampling
    \item learned distribution vs ground truth distribution
    \item closed loop simulator with learned distribution
    \item Monte Carlo sim for probability bound verification
\end{itemize}


\subsection{Hardware}
Show that the assumptions hold in real life (get a cool video). 

\begin{itemize}
    \item shift the controller up to the tx2
    \item put the generative models on the drone with safety filter 
    \item run experiments (don't need to do Monte carlo sim)
\end{itemize}



\clearpage

\section{Method: CVAE's for Dynamics Residual Generative Modeling}

Once trained, a CVAE can be used for estimation of the disturbance's conditional likelihood. Monte Carlo (MC) sampling can be performed to estimate this likelihood as: 
\begin{align}
    p_\theta (\mb{d}|\mb{x}) \approx \frac{1}{S}\sum^S_{s=1} p_\theta (\mb{d} | \mb{x}, \mb{z}^{(s)} ), \quad \mb{z}^{(s)} \sim p_\theta(\mb{z}|\mb{x}). 
\end{align}

Alternatively, the mean and covariance can be directly estimated since the CVAE is parameterized such that $p_\theta(\mb{d}|\mb{x}, \mb{z}) \sim \mathcal{N}(\mu(\mb{x}, \mb{z}), \Sigma(\mb{x}, \mb{z})) $, the MC approximation of the conditional mean and covariance can be calculated as: 
\begin{align}
    \E[\mb{d}|\mb{x}]  & \approx  \frac{1}{S}\left(\sum_{s =1}^S \mu\left(\mb{x}, \mb{z}^{(s)}\right)  \right) \label{eq:mean_approx}\\
    \textup{cov}(\mb{d} | \mb{x}) & \approx \sum_{s=1}^S \frac{1}{S}\left( \Sigma(\mb{x}, \mb{z}^{(s)}) + \mu\left(\mb{x}, \mb{z}^{(s)}\right)\mu\left(\mb{x}, \mb{z}^{(s)}\right)^\top \right) \nonumber\\
    & - \frac{1}{S^2} \left(\sum_{s =1}^S \mu\left(\mb{x}, \mb{z}^{(s)}\right)  \right)\left(\sum_{s =1}^S \mu\left(\mb{x}, \mb{z}^{(s)}\right)  \right)^\top \label{eq:cov_approx}
\end{align}
These calculations consist of neural network forward passes, vector multiplications, and matrix sums and can therefore be very quickly calculated for real-time control. 

==> Old/other_simple_sim_fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/nongaussian.png}
    \caption{The samples from the true distribution are shown in red and plotted over samples from the learned distribution in blue. 10,000 samples from each distribution are drawn and plotted for $x \in \{-3, -1, 1, 3\}$. The overlap of the two distributions shows that our method is capable of learning a non-Gaussian disturbance distribution.}
    \label{fig:nongaussian}
\end{figure}


==> Old/proof_extended_version.tex <==

In this appendix we show that the function \eqref{eq:drone_cbf} is a DTCBF for the Euler approximation of the drone dynamics with the rotation-matrix representation of the system orientation. The effect of using this dynamics representation was analyzed in \cite{tayal_control_2023}.

\begin{proposition}\label{apdx:dtcbf}
    Consider the functions: 
    \begin{align}
        h(\mb{x}) = (C - \bs{\zeta}^\top P \bs{\zeta}) - \lambda (1 - \widehat{\mb{e}}_z \mb{R}\widehat{\mb{e}}_z ), \quad \bs{\zeta} \triangleq \lmat z, & v_z \rmat^\top , \nonumber
    \end{align}
    and: 
    \begin{align}
        \mb{F}_{\textup{Eul}}(\mb{x})  = %\lmat \mb{p}_{k+1} \\ \mb{R}_{k+1} \\ \mb{v}_{k+1} \rmat 
        & \lmat \mb{p} + \Delta_t \mb{v} \\ \mb{R} \\ \mb{v} - \Delta_t g \rmat 
        + \lmat \mb{0} \\
        - \Delta_t \mb{R} [\bs{\omega}]_\times \\ 
     \Delta_t \mb{R} \mb{e}_z \tau \rmat + \lmat \delta_1 \\ \delta_2 \\ \delta_3  \rmat . 
    \end{align}
    with constants $C, \Delta_t, g > 0$, $\mb{e}_z = \lmat 0, & 0, & 1  \rmat^\top $, and $\lambda, \alpha \in [0,1)$ and where $\mb{x} =  \lmat \mb{p}, & \mb{R},& \mb{v}  \rmat^\top \in \R^3 \times SO(3) \times \R^3$ and $\bs{\delta} = \lmat \bs{\delta}_1, & \bs{\delta_2}, & \bs{\delta}_3\rmat^\top \in \R^3 \times \mathfrak{so}(3) \times \R^3$. 
    
    If $C \geq 2 \lambda$ and $P$ satisfies the Discrete-Time Algebraic Ricatti Equation (DARE) for the linear system with 
    \begin{align}
        A = \lmat 1 & \Delta_t \\ 0 & 1  \rmat, \quad  B = \lmat 0 \\ 1\rmat, \\
        Q \in \mathbb{S}^n_{>0}, \quad R \in \mathbb{S}^m_{<0}, \quad (Q - (1 - \alpha) P) \in \mathbb{S}^n_{>0}
    \end{align}
    then there exists $\lmat \tau, & \mb{u} \rmat^\top  \in \R^m$ and $M_{\bs{\delta}}, M_{\bs{c}}>0$ such that 
    \begin{align}
        h(\mb{F}_{\textup{eul}}(\mb{x}, \mb{u}) + \bs{\delta})  + c \geq \alpha h(\mb{x}) 
    \end{align} is feasible for all $  \bs{\delta} < M_\delta,  c < M_c $ and all $\mb{x}$ such that $h(\mb{x}) \geq 0 $. 
\end{proposition}
\begin{proof}
    Let $\varphi(\mb{R}) \triangleq \widehat{\mb{e}}_z^\top \mb{R} \widehat{\mb{e}}_z$.%, then
    % \begin{align}
    %     h(\mb{x}_{k+1})  = &  (C - (A\bs{\zeta} + B \varphi(\mb{R}_k)\tau )^\top P (A\bs{\zeta} + B \varphi(\mb{R}_k) \tau )) \nonumber \\
    %     & - \lambda (1 - \widehat{\mb{e}}_z (\mb{R}_{k} - \Delta_t \mb{R}_{k} [\bs{\omega}]_\times )\widehat{\bs{e}}_z.   
    % \end{align}
    \begin{itemize}
        \item     If $\varphi(\mb{R})  \neq 0 $, then $\tau = \frac{ 1}{\varphi(\mb{R}) } \left( \Delta_t g -  \mb{k}_\textup{DARE}(\bs{\zeta}_k) \right) $ with $[\bs{\omega}]_\times = - \frac{1}{\Delta_t}\delta_3$ yields: 
    \begin{align}
        h(\mb{F}_{\textup{Eul}}(\mb{x}, \mb{u}) + \bs{\delta}) & \geq h(\mb{x}) + \bs{\zeta}^\top Q \bs{\zeta}  - \gamma\left(\left\Vert \lmat \mb{e}_z^\top \bs{\delta_1} \\ \mb{e}_z^\top \bs{\delta_3} \rmat \right\Vert \right)   
    \end{align}
    The inequality comes from using the scaled DARE controller and the existence of $\gamma\in \mathcal{K}$ is guaranteed by the exponential stability nominal system using the DARE controller. Since $(Q - (1 - \alpha) P) \in \mathbb{S}_{>0}^n$ and $R \in SO(3)$, we can expand this inequality as: 
    \begin{align}
        \geq \alpha h(\mb{x}) + (1 - \alpha)( C - 2 \lambda ) -  \gamma\left(\left\Vert \lmat \mb{e}_z^\top \bs{\delta_1} \\ \mb{e}_z^\top \bs{\delta_3} \rmat \right\Vert \right)   
    \end{align}
    Pick $M_{\bs{\delta}} < \gamma^{-1}((1 - \alpha)( C - 2 \lambda )) $ and $M_c \leq (1 - \alpha)(C - 2 \lambda) - \gamma(M_\delta) $, then
    \begin{align}
        h(\mb{F}_{\textup{Eul}}(\mb{x}, \mb{u}) + \bs{\delta}) & \geq \alpha h(\mb{x}) + c
    \end{align}
    
        \item     If $\varphi(\mb{R}) = 0 $, then affect of $\omega$ on $h(\mb{F}_{\textup{Eul}}(\mb{x}, \mb{u}) + \bs{\delta}) $ is 
        \begin{align}
             \lambda \Delta_t \mb{e}_z R [\bs{\omega}]_\times \mb{e}_z =  \mb{e}_z \mb{R}\bs{\varpi} 
        \end{align}        
    % \begin{align}
    %     h& (\mb{F}_{\textup{Eul}}(\mb{x}, \mb{u}) + \bs{\delta})  \nonumber \\
    %     = & (C - \bs{\zeta}_k^\top A^\top P A \bs{\zeta}_k) - \lambda ( 1 - \Delta_t \widehat{\mb{e}}_z\mb{R}_k [\bs{\omega}_k]_\times \widehat{\mb{e}}_z )  \\
    %     = & (C - \bs{\zeta}_k^\top A^\top P A \bs{\zeta}_k) - \lambda(1 - \Delta_t \widehat{\mb{e}}_z \mb{R}_k \bs{\varpi}_k)  
    % \end{align}
    where $\bs{\varpi} = \lmat \omega_x, & \omega_y, & 0 \rmat^\top  $. Since $\varphi(\mb{R}_k) = 0$,  $\mb{e}_z\mb{R}_k $ is perpendicular to $\mb{e}_z$ and thus there exists $\omega_x, \omega_y$ such that: 
        $ h(\mb{x}_{k+1}) = \alpha h(\mb{x}_k) + c $ for any $c \in \R $.
    \end{itemize}



\end{proof}


==> Old/reduced_order.tex <==
\section{Dynamics Learning for Reduced Order Models}

Consider a system with the underlying continuous time dynamics: 
\begin{align}
    \begin{bmatrix}
        \dot{\mb{x}} \\
        \dot{\mb{v}} 
    \end{bmatrix}
    = \begin{bmatrix}
        \mb{v} \\ \mb{a}  
    \end{bmatrix}
\end{align}
If the acceleration is controller by an underlying controller running at a rate faster than $\Delta_t$, then the discrete time dynamics with $v_\textup{des} $ running at a rate of $\Delta_t$ can be written as: 
\begin{align}
    \begin{bmatrix}
        \mb{x}_k \\
        \mb{v}_k
    \end{bmatrix}
    = 
    \begin{bmatrix}
        \mb{x}_k + \Delta_t \mb{v}_k + \frac{1}{2} \Delta_t \overline{\mb{a}}(\mb{e}_k, \mb{v}_\textup{des}) \\
        \mb{v}_k + \Delta_t \overline{\mb{a}}(\mb{e}_k, \mb{v}_{\textup{des}})
    \end{bmatrix} + 
    \begin{bmatrix}
        \bs{\epsilon}_k \\
        \bs{\nu}_k
    \end{bmatrix}
\end{align}
where $\bs{\epsilon}_k \sim \mathcal{E}(\mb{e}_k) $ and $\bs{\nu}_k \sim \mathcal{V}(\mb{e}_k) $ where $\mb{e}$ contains all available state and environment information. 

Consider the case that we are using a single-integrator model for control: 
\begin{align}
    \mb{x}_{k+1} = \mb{x}_{k} + \Delta_t \mb{v}_{k, \textup{des}} + \mb{d}_k (\mb{v}_{k, \des}) 
\end{align}
where $\mb{d}_k \sim \mathcal{D}(\mb{e}_k, \mb{v}_{k, \textup{des}}) $. In this case the disturbance can be written using the current velocity $\mb{v}_k$ and the average acceleration over the time step $\overline{\mb{a}}(\mb{e}_k, \mb{v}_{k, \textup{des}}) $ as: 
\begin{align}
    \mb{d}_k = - \Delta_t (\mb{v}_{k, \textup{des}}  + \mb{v}_k) + \frac{1}{2}\overline{\mb{a}}(\mb{e}_k, \mb{v}_{k, \des}) + \bs{\epsilon}_kk    
\end{align}

If we model the acceleration as an affine function of the desired control input, then this can be written as 
\begin{align}
    \mb{d}_k = - \Delta_t (\mb{v}_{k, \des} + \mb{v}_k) + \frac{1}{2} \Delta_t^2 \bigg( \underbrace{\mb{f}(\mb{e}_k) + \mb{g}(\mb{e}_k) \mb{v}_{k, \des}}_{\overline{\mb{a}}(\mb{e}_k, \mb{v}_{k, \des}  )}  \bigg) + \bs{\epsilon}_k  
\end{align}

The distributions which we want to learn are then: 
\begin{align}
    \mb{b} & \frac{1}{2}\Delta_t^2 f(\mb{e}_k) + \bs{\epsilon}_k \\
    \mb{c} & \mb{g}(\mb{e}_k)
\end{align}
where 
\begin{align}
p (\overline{\mb{a}} | \mb{e}_k, \mb{v}_{k, \des} ) = p(\mb{b} + \mb{c}\mb{v}_{k, \des} | \mb{e}_k, \mb{v}_{k, \des} ).     
\end{align}


\vspace{1em}
\hline 
\vspace{1em}

Consider a system with the discrete update dynamics: 
\begin{align}
    \begin{bmatrix}
        \mb{x}_{k+1} \\
        \mb{v}_{k+1}
    \end{bmatrix} = 
    \begin{bmatrix}
        \mb{x}_k + \Delta \mb{v}_k \\
        \mb{f}(\mb{x}_k, \mb{v}_k) 
    \end{bmatrix}
    + 
    \begin{bmatrix}
        \bs{\epsilon}_k\\ 
        \bs{\nu}_k 
    \end{bmatrix}, \quad 
    \begin{matrix} 
        \bs{\epsilon}_k \sim \mathcal{E} \\
        \bs{\nu}_k   \sim \mathcal{V}
    \end{matrix}
\end{align}
where the system is modeled by the user as 
\begin{align}
    \mb{x}_{k+1} = \mb{x}_k + \mb{d}_k, \quad \mb{d} \sim \mathcal{D} 
\end{align}

We collect a dataset: 
\begin{align}
    D = \left\{ \mb{x}_{k-1}^{(n)}, \mb{x}_{k}^{(n)}, \mb{d}_{k}^{(n)} \right\}_{n=1}^N  
\end{align}
where $\mb{d}_{k}^{(n)} = \mb{x}_{k+1}^{(n)} - \mb{x}_{k}^{(n)} $ which we will use to predict the disturbance distribution for $\mb{d}\sim\mathcal{D}$. 

We can rewrite $\mb{d} $ using the true dynamics: 
\begin{align}
    \mb{x}_0 & = \mb{x}_0 \\
    \mb{x}_1 & = \mb{x}_0 + \Delta_t \mb{v}_0 + \bs{\epsilon}_0 \\
    \mb{x}_2 & = \mb{x}_1 + \Delta_t \mb{v}_1 + \bs{\epsilon}_{1}\\
    &=\mb{x}_1 + \Delta_t \left( \mb{f}(\mb{x}_0, \mb{v}_0) + \bs{\nu}_0  \right) + \bs{\epsilon}_{1}\\
    & = \mb{x}_1 + \Delta_t \left( \mb{f}\left( \mb{x}_0, \frac{\mb{x}_1 - \mb{x}_0 - \bs{\epsilon}_0 }{\Delta_t }\right) + \bs{\nu}_0  \right) + \bs{\epsilon}_1 
\end{align}

\subsection{Reduced order model}

Consider the case where the disturbance distribution is non-Markovian and depends on the entire state history: 
\begin{align}
    \mb{d} \sim p(\mb{d} ~|~ \mb{x}_{k:0}) 
\end{align}
Given this non-Markovian nature of the true distribution, the learned distibution approximates: 
\begin{align}
    p_\theta(\mb{d}|\mb{x}_{k}) \approx \int_{\Pi^k R^n} p(\mb{d} | \mb{x}_{k:0}) p(\mb{x}_{k-1:0})  d\mb{x}
\end{align}
In this way the learned distribution can capture non-Markovian effects present in the data. 

\clearpage
